Hierarchical Autoregressive Transformers: Combining Byte- and Word-Level Processing for Robust, Adaptable Language Models

Tokenization is a fundamental step in natural language processing, breaking text into units that computational models can process. While learned subword tokenizers have become the de-facto standard, they present challenges such as large vocabularies, limited adaptability to new domains or languages, and sensitivity to spelling errors and variations. To overcome these limitations, we investigate a hierarchical architecture for autoregressive language modelling that combines character-level and word-level processing. It employs a lightweight character-level encoder to convert character sequences into word embeddings, which are then processed by a word-level backbone model and decoded back into characters via a compact character-level decoder. This method retains the sequence compression benefits of word-level tokenization without relying on a rigid, predefined vocabulary. We demonstrate, at scales up to 7 billion parameters, that hierarchical transformers match the downstream task performance of subword-tokenizer-based models while exhibiting significantly greater robustness to input perturbations. Additionally, during continued pretraining on an out-of-domain language, our model trains almost twice as fast, achieves superior performance on the target language, and retains more of its previously learned knowledge. Hierarchical transformers pave the way for NLP systems that are more robust, flexible, and generalizable across languages and domains.

==> tables/splitting_0.tex <==
\resizebox{\textwidth}{!}{
\begin{footnotesize} 
\begin{tabular}{l|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c}
% \toprule
Model & \rotatebox{90}{DCLM Acc} & \rotatebox{90}{MMLU} & \rotatebox{90}{LBD OAI} & \rotatebox{90}{LBD OAI C} & \rotatebox{90}{LBD} & \rotatebox{90}{LBD C} & \rotatebox{90}{LBD OAI MT} & \rotatebox{90}{ARC C} & \rotatebox{90}{ARC E} & \rotatebox{90}{OpenBook QA} & \rotatebox{90}{TriviaQA} & \rotatebox{90}{TFQA MC1} & \rotatebox{90}{TFQA MC2} & \rotatebox{90}{WinoGr} & \rotatebox{90}{HellaSwag} & \rotatebox{90}{WiC} & \rotatebox{90}{WebQs} & \rotatebox{90}{PIQA} & \rotatebox{90}{BoolQ} & \rotatebox{90}{XNLI} \\
\midrule \hline
\textbf{1B} &&&&&&&&&&&&&&&&&&&& \\ \hline
Whitespace Splitter & \textbf{83.7} & \textbf{26.0} & \textbf{64.6} & \textbf{8.8} & \textbf{56.5} & \textbf{3.3} & \textbf{64.6} & \textbf{30.5} & \textbf{65.0} & \textbf{24.8} & \textbf{9.6} & 22.3 & 35.9 & \textbf{61.4} & \textbf{46.5} & \textbf{54.7} & \textbf{4.0} & \textbf{73.0} & \textbf{60.2} & \textbf{37.5} \\ \hline
Fixed Splitter & 82.6 & 25.9 & 57.3 & 2.1 & 48.1 & 0.6 & 57.3 & 28.2 & 62.8 & 21.0 & 5.1 & 21.8 & 36.3 & 56.9 & 43.8 & 48.1 & 2.6 & 69.6 & 58.2 & 34.1 \\ \hline
Megabyte & 80.0 & 25.1 & 51.3 & 2.1 & 41.0 & 0.7 & 51.3 & 23.4 & 54.9 & 20.2 & 2.9 & \textbf{23.3} & \textbf{38.1} & 53.0 & 38.9 & 52.0 & 1.5 & 68.8 & 55.8 & 34.4 \\ \hline
\bottomrule
\end{tabular}
\end{footnotesize}
}
